3DIoUMatch: Leveraging IoU Prediction for Semi-Supervised 3D Object Detection

3D object detection is an important yet demanding task that heavily relies on difficult to obtain 3D annotations. To reduce the required amount of supervision, we propose 3DIoUMatch, a novel semi-supervised method for 3D object detection applicable to both indoor and outdoor scenes. We leverage a teacher-student mutual learning framework to propagate information from the labeled to the unlabeled train set in the form of pseudo-labels. However, due to the high task complexity, we observe that the pseudo-labels suffer from significant noise and are thus not directly usable. To that end, we introduce a confidence-based filtering mechanism, inspired by FixMatch. We set confidence thresholds based upon the predicted objectness and class probability to filter low-quality pseudo-labels. While effective, we observe that these two measures do not sufficiently capture localization quality. We therefore propose to use the estimated 3D IoU as a localization metric and set category-aware self-adjusted thresholds to filter poorly localized proposals. We adopt VoteNet as our backbone detector on indoor datasets while we use PV-RCNN on the autonomous driving dataset, KITTI. Our method consistently improves state-of-the-art methods on both ScanNet and SUN-RGBD benchmarks by significant margins under all label ratios (including fully labeled setting). For example, when training using only 10\% labeled data on ScanNet, 3DIoUMatch achieves 7.7% absolute improvement on mAP@0.25 and 8.5% absolute improvement on mAP@0.5 upon the prior art. On KITTI, we are the first to demonstrate semi-supervised 3D object detection and our method surpasses a fully supervised baseline from 1.8% to 7.6% under different label ratios and categories.

==> [CVPR 21] 3DIoUMatch/tex/00_abstract.tex <==
\begin{abstract}
% version 2.1
3D object detection is an important yet demanding task that heavily relies on difficult to obtain 3D annotations. To reduce the required amount of supervision, we propose 3DIoUMatch, a novel semi-supervised method for 3D object detection applicable to both indoor and outdoor scenes.
We leverage a teacher-student mutual learning framework to propagate information from the labeled to the unlabeled train set in the form of pseudo-labels. 
However, due to the high task complexity, we observe that the pseudo-labels suffer from significant noise and are thus not directly usable. 
To that end, we introduce a confidence-based filtering mechanism, inspired by FixMatch. 
We set confidence thresholds based upon the predicted objectness and class probability to filter low-quality pseudo-labels.
While effective, we observe that these two measures do not sufficiently capture localization quality. 
We therefore propose to use the estimated 3D IoU as a localization metric and set category-aware self-adjusted thresholds to filter poorly localized proposals.
We adopt VoteNet as our backbone detector on indoor datasets while we use PV-RCNN on the autonomous driving dataset, KITTI.
%The key to our approach is a novel differentiable 3D IoU estimation module. This module is used for filtering poorly localized proposals as well as for IoU-guided bounding box deduplication. 
%At inference time, this module is further utilized to improve localization through test-time optimization. 
Our method consistently improves state-of-the-art methods on both ScanNet and SUN-RGBD benchmarks by significant margins under all label ratios (including fully labeled setting). 
For example, when training using only 10\% labeled data on ScanNet, 3DIoUMatch achieves 7.7\% absolute improvement on mAP@0.25 and 8.5\% absolute improvement on mAP@0.5 upon the prior art. 
On KITTI, we are the first to demonstrate semi-supervised 3D object detection and our method surpasses a fully supervised baseline from 1.8\% to 7.6\% under different label ratios and categories.



% Version 2.0
% 3D object detection is an important and demanding task that heavily relying on expensive 3D annotation.
% To reduce the amount of supervision, we propose 3DIoUMatch, a novel method for semi-supervised 3D object detection.
% In this work, we adopt VoteNet, a popular point cloud based object detector, as our backbone and leverage a teacher-student mutual learning framework that propagates pseudo-labels from a teacher model to a learnable student model.
% We observe that the pseudo-labels are highly noisy due to the difficulty of 3D object detection task, which significantly hampers the semi-supervised learning.
% To improve pseudo-label quality, we set confidence thresholds based upon the predicted objectness and class probabilty to filter low-quality pseudo-labels.
% While effective, we observe that these two measures do not sufficiently capture localization quality. 
% To that end, we for the first time propose to incorporate IoU prediction as a localization confidence for pseudo-label filtering, and devise the first differentiable 3D IoU estimation module, which further enables 3D IoU-guided NMS and 3D IoU optimization.
% %A recent approach, SESS, has demonstrated promising results by promoting consistency between the predictions of a student and a teacher model.  
% %Inspired by advances in semi-supervised learning, we extend SESS by incorporating an object proposal filtering mechanism based on objectness score and class probability. 
% Our method consistently improves state-of-the-art methods on both ScanNet and SUN-RGBD benchmarks by significant margins. 
% For example, when training using only 10\% label data on ScanNet, 3DIoUMatch achieves XX absolute improvement on mAP@0.25 and XX absolute improvement on mAP@0.5.
% Larger improvements are attained with less supervision. 


%For example, when training with only 10\% labeled data we get 8\% and 7\% on mAP@0.5 on both ScanNet and SUN-RGBD dataset, respectively. Larger improvements are attained with less supervision. 

% In this work, we propose 3DIoUMatch, a novel method for semi-supervised 3D object detection(SS-3DOD). Previous work on SS-3DOD simply leverages consistency regularization between the outputs from a student model and a teacher model.
% Inspired by several SS-OD works on 2D images, we incorporate confidence-based filtering mechanism into our framework, where a confidence threshold on objectness and top-1 class probability is applied to filter low-quality bounding box.
% We observe that these two confidences don't sufficiently capture localization quality, so we propose to additionally filter with a localization confidence, which is the estimated 3D IoU of a bounding box prediction. 
% We devise the first differentiable 3D IoU branch that can support both IoU prediction and test-time IoU optimization. 
% Instead of naively using a constant IoU threshold for bounding box filtering, we propose lower-half suppression (LHS) technique to suppress the redundant bounding boxes predictions from teacher models while yielding a self-adjusted class-aware IoU threshold.
% Our method consistently improved state-of-the-art
% methods by significant margins, 7\% and 3\% on mAP@0.25 and 8\% and 7\% on mAP@0.5 on both ScanNet and SUN-RGBD dataset,respectively, when training with 10\% labeled data. When training with only 5\% labeled data, our method improves even more.




\end{abstract}

==> [CVPR 21] 3DIoUMatch/tex/01_intro.tex <==
\blfootnote{*: equal contribution}
\blfootnote{Project page:~\href{http://THU17cyz.github.io/3DIoUMatch}{http://THU17cyz.github.io/3DIoUMatch}}
Object detection is a key task in 3D scene understanding. It provides a concise representation of raw sensor measurements in the form of semantically meaningful 3D bounding boxes. This low-dimensional representation can already serve numerous applications in autonomous driving and AR/VR, as well as in robot navigation and manipulation.  As a result, in recent years there has been a surge of interest in developing improved object detection pipelines and indeed current state-of-the-art methods show impressive performance. Yet, much of their success is attributed to the availability of large datasets of 3D scenes that are carefully annotated. While rapid advances in sensor technology facilitate the collection of 3D scenes at scale, annotating them remains the main bottleneck. This calls for detection methods that can leverage both labeled and unlabeled data at train time. 

In this work, we aim to address this requirement by proposing a novel semi-supervised 3D object detection method which we dub 3DIoUMatch. 
As a generally applicable method, 3DIoUMatch can be applied to both indoor scene datasets, \textit{i.e.} ScanNet\cite{dai2017scannet} and SUN-RGBD\cite{song2015sun}, and outdoor datasets,  \textit{i.e.} KITTI\cite{geiger2013vision}. We adopt popular point-based object detectors, VoteNet~\cite{qi2019deep} and PV-RCNN~\cite{shi2020pv}, as our backbone object detection networks for the indoor and outdoor scenes, correspondingly.
%As our backbone object detection network we adopt VoteNet~\cite{qi2019deep}, a popular point-based object detector\yezhen{for indoor 3D detection, and PV-RCNN~\cite{shi2020pv} for outdoor 3D detection}. 
To provide supervision to the unlabeled scenes, we leverage a teacher-student mutual learning framework~\cite{tarvainen2017mean} and use the bounding box predictions from the teacher network as pseudo-labels to supervise the student network on unlabeled data. 
However, unlike most pseudo-label techniques that were designed for classification, in the highly complex (joint regression and classification) task of object detection, we observe that the pseudo-labels suffer from significant noise, and using them directly is suboptimal.  

Inspired by FixMatch~\cite{sohn2020fixmatch}, the state-of-the-art semi-supervised learning (SSL) method for 2D image classification that proposed confidence-based filtering to improve pseudo-label quality, we adopt a pseudo-label filtering mechanism for 3D object detection by setting thresholds on predicted class probabilities (and objectness scores for VoteNet), so as to filter out teacher proposals with potentially erroneous semantic labels or ones not belong to foreground. 
%This is not needed now -- 
%This filtering mechanism ensures that only highly-confident pseudo-labels will be passed to supervise the student network.
%that only passes teacher label predictions with high class-probability and objectness score to supervise the student network. 
While effective, these criteria alone are not sufficient to capture localization quality, and the pseudo-labels may still have large errors in the bounding box parameters. To that end, we further propose to leverage estimated IoU (intersection over union) as a localization quality measure for pseudo-label filtering. IoU estimation was first proposed in the context of 2D object detection as a localization confidence in the pioneering work IoU-Net~\cite{jiang2018acquisition}, where estimated IoU was proven successful in replacement of class confidence for test-time Non-Maximal Suppression (NMS).
%Here, we propose to leverage predicted IoU for pseudo-label filtering on object detection tasks. 
To the best of our knowledge, leveraging IoU estimation for pseudo-label filtering is a novel idea for SSL on both 2D and 3D object detection. %\yezhen{While PV-RCNN is equipped with an IoU estimation module, VoteNet lacks such a structure, and we devised a differentiable 3D IoU estimation module for VoteNet. With the help of these IoU modules, we are able to filter out poorly localized pseudo-labels and leverage estimated IoU for both train-time and test-time NMS.} \verify{With our newly devised differentiable 3D IoU estimation module, we are able to filter out poorly localized pseudo-labels and leverage estimated IoU for both train-time and test-time NMS. }
Equipping the detectors with a 3D IoU estimation module, we are able to filter out poorly localized pseudo-labels and leverage estimated IoU for both train-time and test-time NMS.
%With the capability of estimating 3D IoU, we have two experimental findings: 1) at training time, IoU-guided NMS is helpful to further reduce the redundancy in pseudo-labels. However, we find that suppressing half of the highly-overlapping boxes is more robust than all but the top few, due to limited accuracy of 3D IoU estimation. We coin this new suppression method \textit{Lower-Half Suppression}(LHS); 2) at test time, our 3D IoU module can perform IoU optimization that refines the bounding box parameters. We note that this is not possible with the non-differentiable IoU module proposed in\cite{yang2019std}.

A key challenge when filtering based on IoU estimation is how to properly set the threshold. Unlike objectness and class confidence for which high threshold values (e.g. 0.9) work well, 3D IoU is more sensitive to small errors. Setting the threshold too high would reduce the number of pseudo-labels to very few, from which little could be learned. To balance between quality and coverage, we propose a two-stage filtering process: first, using a relatively low IoU threshold; then, an IoU-guided class-aware \textit{Lower-Half Suppression} (LHS) that removes only half of the highly-overlapping boxes with low predicted IoU. Our proposed LHS thus naturally sets a threshold that is both dynamic and class-aware. Our experiments show that LHS outperforms IoU-guided NMS, which suppresses all but the top one during semi-supervised training. 
%\verify{Beyond train-time filtering, we also leverage our differentiable 3D IoU module for test-time IoU-guided NMS and optimization-based bounding box refinement, which is not possible with previous non-differentiable 3D IoU modules~\cite{yang2019std}.}

% \orl{Key to our approach is thus a newly devised differentiable 3D IoU estimation module which we use for filtering poorly localized proposals. At inference time, this module is further utilized for refining the bounding box parameters through test-time IoU optimization.  }
Our method consistently improves upon the previous state-of-the-art method, SESS~\cite{zhao2020sess}, on both ScanNet and SUN-RGBD benchmarks by significant margins. When using only 10\% labeled data on ScanNet, 3DIoUMatch outperforms SESS by 7.7 absolute improvement on mAP@0.25 and by 8.5 absolute improvement on mAP@0.5. When using 5\% labeled data on SUN-RGBD, 3DIoUMatch outperforms SESS by 4.8 absolute improvement on mAP@0.25 and by 8.0 absolute improvement on mAP@0.5. 
%\yezhen{On KITTI, since we are the first outdoor 3D detection work, we only compare with the fully-supervised baseline, which we also surpass by a large margin under different label ratios.}
On KITTI, we are the first to demonstrate semi-supervised 3D object detection work and surpass fully-supervised baseline by large margins under all label ratios.

Our main contributions can be summarized as follows:
\begin{enumerate}
    \myitem We propose a novel semi-supervised method for 3D object detection in point clouds based on pseudo-label propagation along with a carefully designed filtering mechanism. 
    \myitem For the first time, we leverage predicted 3D IoU as a localization confidence score for pseudo-label filtering, and further propose IoU-guided Lower-Half Suppression for robust pseudo-label deduplication. This idea is generally applicable and can be coupled to different 3D detectors on both indoor and outdoor scenes.
    %\myitem Key to our approach is the usage of estimated 3D IoU as a localization confidence for pseudo-label filtering, and to guide bounding-box lower-half suppression.
    %\he{Just want to double check with or.  Shouldn't we emphasize the "for-the-first-time" novelty of using IoU as confidence metric?}
    % \myitem We devise a novel 3D IoU prediction module that enables localization filtering, test-time IoU-guided NMS, and bounding box refinement.
    %\he{I would prefer to highlight that we propose to use 3D IoU for filtering instead of saying that the newly devised 3D IoU module is the main contribution.}
    %\myitem We devise a \yezhen{differentiable} 3D IoU module \yezhen{for point-cloud-based networks like VoteNet} that enables our localization filtering, IoU-guided bounding box suppression, and IoU optimization for bounding box refinement.
    %
    \myitem We achieve markedly improved performance over the previous state-of-the-art semi-supervised 3D object detection methods on the two major indoor object detection benchmarks, ScanNet and SUN-RGBD, under low label ratios and fully labeled setting. As the first semi-supervised 3D object detection work on KITTI, we also achieve significant improvements compared to fully supervised method.
    %\yezhen{, and also on one outdoor object detection benchmark, KITTI}.
\end{enumerate}


 

% Reduce supervision for 3D object detection is important.

% \textbf{Main contributions:}
% \begin{enumerate}
%     \item We design a principled SSL method for 3D object detection. To that end we propose to filter teacher predictions as well as careful association.
%     \item We further introduce a localization mechanism in the form of a 3D-IoU prediction module. Importantly, our module is differentiable and allow filtering as well as test-time-refinement. 
%     \item Compared with its predecessor, 3DIoUMatch achieves markedly improved performance across different label ratio and on both benchmarks.
% \end{enumerate}

==> [CVPR 21] 3DIoUMatch/tex/02_related.tex <==
\begin{figure*}[t]
\begin{center}
   \includegraphics[width=0.8\linewidth]{figure/ssl_new.pdf}
\end{center}
   \caption{\textbf{3DIoUMatch pipeline at semi-supervised training stage.} We adopt as our backbone an extended version of VoteNet with an additional 3D IoU estimation module. For SSL, we utilize a teacher-student mutual learning framework, composed of a learnable student taking strongly augmented input data and an EMA teacher taking weakly augmented input samples. On labeled data, the student network is supervisedly trained. On unlabeled data, the student network takes pseudo-labels from its EMA teacher. To improve the quality of pseudo-label, we adopt a confidence-based filtering mechanism that filters out predictions that fail to pass all thresholds on class probability, objectness, and 3D IoU. We further use IoU-guided Lower-Half Suppression to remove the duplicated predictions. Using the filtered pseudo-labels, we selectively supervise the student predictions that are around the bounding boxes in the pseudo-labels.}
\label{fig:long}
\end{figure*}

\paragraph{Semi-Supervised Learning (SSL)}
Many of the recent SSL methods~\cite{berthelot2019mixmatch, xie2019unsupervised, berthelot2019remixmatch} leverage consistency regularization, first proposed in \cite{sajjadi2016regularization, laine2016temporal}, which enforces the model to predict consistently across label-preserving data augmentation of different intensity. Borrowing the concept from Mean Teacher~\cite{tarvainen2017mean}, the model with frozen weight can be viewed as the teacher model, otherwise student model. Some methods~\cite{berthelot2019mixmatch}, following Mean Teacher, make the teacher model as the EMA of the student model for further regularization. Pseudo labeling~\cite{lee2013pseudo} is another popular class of SSL method which can also be treated as a kind of consistency regularization, as one output of the unlabeled data is enforced to be consistent with the other (the pseudo-labels) by being supervised with the other. To improve the quality of pseudo-labels, FixMatch~\cite{sohn2020fixmatch}, a state-of-the-art SSL work on image classification, has shown that the student network can improve significantly by setting a classification confidence threshold $\tau_{cls}$ and filtering out low-confidence predictions from the teacher. With the filtered pseudo-labels, the student model only gets supervised on the unlabeled data whose pseudo-labels are kept. Another key factor to the success of these methods is strong data augmentation. It has been shown crucial to many SSL works~\cite{sajjadi2016regularization, laine2016temporal, xie2019unsupervised}. Recent works~\cite{berthelot2019remixmatch, sohn2020fixmatch} proposed to adopt even more powerful augmentation such as RandAugment~\cite{cubuk2020randaugment} and Cutout~\cite{devries2017improved}.
%Under the teacher-student framework, feeding strongly-augmented and therefore harder input to the student model guarantees the relatively better performance of the teacher model. 

\mypara{Semi-Supervised Object Detection}
Since the beginning of the deep learning era, tremendous progress has been made in 2D object detection, e.g region-based detectors~\cite{girshick2014rich, girshick2015fast, ren2015faster} and single-stage detectors~\cite{liu2016ssd, redmon2016you, tian2019fcos}. Similarly in 3D object detection, a number of deep learning methods have been proposed for different 3D data modalities, e.g. RGBD-based detectors~\cite{qi2018frustum,qi2020imvotenet}, point-based detectors~\cite{yi2019gspn, shi2019pointrcnn, lang2019pointpillars, qi2019deep}, voxel-based detectors~\cite{zhou2018voxelnet}, point-voxel-based detectors~\cite{shi2020pv}, etc.

Despite the great progress in both 2D and 3D object detection, most works focused on a fully-supervised setting. A few works~\cite{hoffman2014lsda, gao2019note} have proposed to leverage unlabeled data or weakly-annotated data for 2D object detection. 
%Under a weakly-supervised setting, LSDA\cite{hoffman2014lsda} and NoteRCNN\cite{gao2019note} leverages training data only with image-level annotation.
Under a standard SSL setting as we follow, CSD~\cite{jeong2019consistency} proposed a consistency regularization method to enforce the consistency between predictions from an image and its flipped version. STAC~\cite{sohn2020simple} adopts a two-stage scheme for training Faster R-CNN~\cite{ren2015faster}: in the first stage it pre-trains a detector with labeled data only and then predicts the pseudo labels for the unlabeled data; in the second stage, STAC leverages asymmetric data augmentation and the pseudo-label filtering mechanism to remove object proposals with low confidence. Note that the pseudo-labels are only generated once at the end of the first stage. 
%inspired by FixMatch\cite{sohn2020fixmatch},  filters the pseudo labels by setting a threshold on confidence score and only supervise the detector on unlabeled data. STAC also introduces stronger data augmentation for object detection. 
% \he{not sure if we need to cite}The most closely relevant work to us is unbiased Teacher\cite{anonymous2021unbiased}, which also leverage use a teacher-student mutual learning framework and focal loss to alleviate class imbalance issue. 

The only prior work on semi-supervised point-based 3D object detection, is SESS~\cite{zhao2020sess}. SESS is built upon VoteNet~\cite{qi2019deep} and adopts a two-stage training scheme. It leverages a mutual learning framework composed of an EMA teacher and a student, uses asymmetric data augmentation, and enforces three kinds of consistency losses between the teacher and student outputs. Although SESS brings noticeable improvements upon a vanilla VoteNet when using only a small portion of labeled data, we find their consistency regularization suboptimal, as it is uniformly enforced on all the student and  teacher predictions. In this work, we instead propose to apply confidence-based filtering to improve the quality of pseudo-labels from the teacher predictions and we are the first (in both 2D and 3D object detection) to introduce IoU estimation for localization filtering. 

\mypara{IoU Estimation}
IoU estimation was first proposed in a 2D object detection work IoU-Net~\cite{jiang2018acquisition}, which proposed an IoU head that runs in parallel to bounding box refinement and is differentiable w.r.t. bounding box parameters. IoU-Net adds an IoU estimation head to several off-the-shelf 2D detectors and uses IoU estimation instead of classification confidence to guide NMS, which improves the performance consistently over different backbones. Thanks to its differentiability, IoU-Net can perform IoU optimization on bounding box parameters for iterative refinement, which further brings noticeable performance improvement.

%The differentiable IoU module proposed in IoU-Net crops RoI features using predicted bounding box from RPN feature map and perform a Precise RoI Pooling followed by a MLP for 2D IoU prediction.
% IoU-Net\cite{jiang2018acquisition} proposed a differentiable IoU module that crops RoI features using predicted bounding box from RPN feature map and perform a Precise RoI Pooling followed by a MLP for 2D IoU prediction.
%cropping RoI features using predicted bounding box from RPN feature map and performing a Precise RoI Pooling followed by an MLP for 2D IoU prediction. Because of the regularity of 2D feature maps, with Precise RoI Pooling IoU-Net can interpolate the feature map continuously and takes the integral of the RoI, which makes the IoU estimation continuously differentiable.

%Then IoU-Net proposes iteratively refining bounding box parameters, namely IoU optimization, with gradient ascent by viewing the IoU estimation as an optimization objective. Applying IoU optimization also brings consistent improvement to different network backbones equipped with the IoU estimation head.
% With the computed gradient, IoU-Net tries to maximize the IoU estimation between the detected bounding box and its matched ground-truth, and
% Moreover, IoU-Net proposes Precise RoI Pooling in replacement of RoIAlign in order that IoU estimations are continuously differentiable w.r.t. bounding box coordinates, which enables the test-time IoU optimization. 
For 3D object detection, STD~\cite{yang2019std} follows IoU-Net to add a simple IoU estimation branch parallel with the box estimation branch and to guide NMS with IoU estimation. 
PV-RCNN~\cite{shi2020pv} devises a similar 3D IoU estimation module and use it at IoU-guided NMS stage. These two modules, unfortunately, are not suitable for IoU optimization as the features fed to the IoU estimation branch are not differentiable w.r.t. the bounding box size.
Since the original VoteNet is not equipped with an IoU module, we devise a differentiable point-cloud-based 3D IoU estimation module is simple yet effective that can support the IoU optimization.
%This IoU estimation module design, unfortunately, is not suitable for IoU optimization as the features fed to the IoU estimation branch are not differentiable w.r.t. the bounding box size. This is because STD concatenates the canonical coordinates w.r.t. box center with features of interior points to create the initial features for each bounding box proposal, which is unaware of the box size. Moreover, the bounding box location is regressed along with IoU estimation so the bounding box estimated and optimized is the one before regression, namely the feature offset problem~\cite{zhu2019iou}, which is also a problem in IoU-Net. \yezhen{The IoU module in PV-RCNN~\cite{shi2020pv} also has the similar problem.}
% 3D IoU-Net\cite{li20203d} designs a much more complicated IoU estimation module and solves the feature offset problem yet the IoU estimation is still not differentiable w.r.t. box size and angle.         I find 3D IoU-Net is actually differentiable, but just because of concatenated xyzs, so it's not THAT differentiable
%In contrast, our \yezhen{point-cloud-based} 3D IoU estimation module is simple yet effective, can support the IoU optimization while avoiding the feature offset problem. 

% \he{Yezhen: How PV-RCNN implements its 3D IoU estimation module?}
% \yezhen{PV-RCNN predicts the IoU of each proposal with its RoI-grid pooling module, which divides each RoI into grids and aggregates the information of each grid with set abstractions operations.}
%and the feature offset problem is avoided since VoteNet do not have a bounding box refinement step and the devised IoU module is not parallel with, but after, the box proposal module of VoteNet. By leveraging the IoU estimations during test time as IoU-Net, our method further improves the performance by a large margin. 


==> [CVPR 21] 3DIoUMatch/tex/03_method.tex <==
In this section, we describe our solution in detail. We first formulate our problem in \ref{sec:formulation} and then summarize the two object detection backbones, PV-RCNN and VoteNet, in \ref{sec:votenet}. We use VoteNet as an example to illustrate our proposed 3DIoUMatch pipeline in \ref{sec:pipeline}. We further explain how we use the estimated 3D IoU for pseudo-label filtering and deduplication in \ref{sec:pseudo-label}. Finally, we illustrate how we leverage the pseudo-labels for supervision in \ref{sec:supervise}.
%since our backbone detection module is based on VoteNet, we summarize it in \ref{sec:votenet}. We then explain our newly devised 3D IoU estimation module in \ref{sec:iou-module}. 
%These set the stage for a detailed description of our proposed 3DIoUMatch pipeline in \ref{sec:pipeline}. We further explain how we use the estimated 3D IoU for pseudo-label filtering and deduplication in \ref{sec:pseudo-label}. Finally, we illustrate how we leverage the pseudo-labels for supervision in \ref{sec:supervise}.


\subsection{Problem Definition}\label{sec:formulation}
Given a 3D point cloud representation of a scene $\boldsymbol{x} \in \mathbb{R}^{N\times 3}$ containing a set of objects $O = \{o^{(j)}\}$, we aim at detecting the amodal oriented 3D bounding boxes of all objects in $O$, along with their semantic class labels. In particular, we are interested in accomplishing this task under challenging conditions of limited supervision
%
%In this work, our objective is to address 3D object detection in a semi-supervised setting,
% 
where we have access to a (small) set of labeled scenes $\{\boldsymbol{x}^l_i, \boldsymbol{y}^l_i\}_{i=1}^{N_l}$ and a set of unlabeled scenes $\{\boldsymbol{x}^u_i\}_{i=1}^{N_u}$, where $N_l$ and $N_u$ are the number of labeled and unlabeled scenes, respectively. For a labeled scene $\boldsymbol{x}$, the label $\boldsymbol{y}$ comprises bounding box parameters $\{\boldsymbol{b}^{(j)}\}$ and semantic class labels $\{q^{(j)}\}$ of all ground truth objects $\{o^{(j)}\}$. 




\subsection{IoU-aware 3D Object Detection}
\label{sec:votenet}
%\he{Describe VoteNet and PV-RCNN, start with their common settings, then their differences (for VoteNet, mention that we incorporate an IoU Module and refer to supp.) Optional: in supp, describe PV-RCNN like what you did here for VoteNet.}
%\yezhen{
% 3D object detection can be categorized as indoor detection and outdoor detection. VoteNet \cite{qi2019deep}, is a popular single-stage object detector for indoor 3D point clouds. PV-RCNN is a two-stage object detection for outdoor point clouds.}
We experiment our SSL method on two 3D detectors, VoteNet \cite{qi2019deep} and PV-RCNN \cite{shi2020pv}. VoteNet is a single-stage indoor point cloud detector while PV-RCNN is a two-stage outdoor point cloud detector. They both take point clouds only for inputs and output a list of bounding boxes after Non-Maximum Suppression (NMS) for each scene, which contain the prediction of center, size, orientation and semantic class. However, their architecture are very different partly due to the great discrepancy between indoor and outdoor scenes.

\noindent\textbf{Indoor scene detector: VoteNet} VoteNet \cite{qi2019deep} is built upon PointNet++~\cite{qi2017pointnet++} backbone, and first processes the input point cloud $\{x_i\}_{i=1}^{N}$ to generate a sub-sampled set of $M < N$ seed points enriched with high-dimensional features $\{[x_i;f_i]\in\mathbb{R}^{3+C}\}_{i=1}^{M}$.
%where $x_i\in\mathbb{R}^{3}$, and $f_i\in\mathbb{R}^{C}$. 
Next, each seed point votes for the center of the object it belongs to, and the votes are grouped into $K$ clusters. Finally, each of the K vote clusters is aggregated to make a prediction of a 3D bounding box parameters $\boldsymbol{b}^{(k)}$, a corresponding objectness score $s_k = \text{P}(\boldsymbol{b}^{(k)}~ \text{is an object})$, %to indicate whether or not the vote cluster is in the vicinity of an object,\he{Not sure if this is clear}\orl{is this better?}, 
and a probability distribution $\{p_{cls}\}$ over $L$ possible semantic classes. 
%\orl{maybe this? $p_{cls}^{(k)} \in {[0,1]}^L$}
The bounding box parameters $\boldsymbol{b}$ are its center location $\mathbf{c} \in \mathbb{R}^{3}$, scale $\mathbf{d}\in \mathbb{R}^{3}$, and orientation $\theta$ around the upright axis.

At train time, VoteNet jointly minimizes a weighted combination of the following target losses: vote coordinate regression, objectness score binary classification, box center regression, bin classification and residual regression for heading angle, scale regression, and category classification. At test time, VoteNet applies Non-Maximum Suppression (NMS) based on objectness score to remove duplicated bounding boxes. Here, we instead rely on a 3D IoU estimation module designed for VoteNet. For more details, refer to the supplementary materials.
%We then explain our newly devised 3D IoU estimation module in \ref{sec:iou-module}. 

\noindent\textbf{Outdoor scene detector: PV-RCNN} PV-RCNN\cite{shi2020pv} is a high-performance and efficient LiDAR point cloud detector that deeply integrates both 3D voxel CNNs and PointNet++-style set abstraction to learn more discriminative point cloud features. Specifically, PV-RCNN first passes the 3D scene through a novel voxel set abstraction module based on sparse 3D CNN to get a set of keypoints with representative scene features. Then RoI grid pooling is then applied to the keypoints to abstract proposal-specific features into RoI grid points. The RoI grid points containing rich context information are finally used to accurately estimate bounding box parameters.

PV-RCNN itself incorporates an IoU-estimation module which can predict the IoU of each bounding box and use it to guide the sorting of the boxes. 

 
\subsection{3DIoUMatch for SSL on 3D object detection}\label{sec:pipeline}
%\yezhen{We take VoteNet as our example and our method with PV-RCNN is similar}. 
We take VoteNet as our example and our method with PV-RCNN is similar.
With the incorporation of 3D IoU module into VoteNet, we construct an IoU-aware VoteNet for SSL on 3D object detection. Our proposed solution is comprised of two training stages:  a pre-training stage, where we train our IoU-aware VoteNet on the labeled data, followed by an SSL stage where the entire data is utilized by pseudo-labeling the unlabeled scenes.

\mypara{Pre-training.} We start by training our IoU-aware VoteNet in a supervised manner, using the labeled set $\{\boldsymbol{x}^l_i, \boldsymbol{y}^l_i\}_{i=1}^{N_l}$. The training loss is a sum over the original VoteNet losses $L_\text{votenet}$ and 3D IoU loss $L_\text{IoU}$. Once converged, we clone the network to create a pair of student and teacher networks. 

\mypara{Semi-supervised training through a teacher-student framework.}
We follow a teacher-student mutual learning framework~\cite{tarvainen2017mean} and train our networks on both labeled $\{\boldsymbol{x}^l_i, \boldsymbol{y}^l_i\}_{i=1}^{N_l}$ and unlabeled data $\{\boldsymbol{x}^u_i\}_{i=1}^{N_u}$. Each training batch contains a mixture of $\{\boldsymbol{x}^l_i\}_{i=1}^{B_l}$ labeled samples and $\{\boldsymbol{x}^u_i\}_{i=1}^{B_u}$ unlabeled samples. %, where $B_l$ and $B_u$ represent the number of the labeled and unlabeled samples in a batch, correspondingly.

For labeled samples, we supervise the student network using ground truth supervisions (as done in the pre-training stage) whereas for unlabeled samples, the student networks is supervised using pseudo-labels $\{\boldsymbol{\tilde{y}}^u_i\}_{i=1}^{N_u}$ generated
from the teacher network. The final loss is formed as:
$$ L = L_{l}(\{\boldsymbol{x}^l_i\}_{i=1}^{N_l}, \{\boldsymbol{y}^l_i\}_{i=1}^{N_l}) + \lambda_{u}L_{u}(\{\boldsymbol{x}^u_i\}_{i=1}^{N_u},\{\boldsymbol{\tilde{y}}^u_i\}_{i=1}^{N_u}) $$ where $\lambda_{u}$ is the unsupervised loss weight.

To succeed in semi-supervised learning, it is crucial for the teacher network to generate high-quality pseudo-labels and maintain a reliable performance margin over the student network throughout the training. As commonly used in SSL literature, e.g. Mean Teacher~\cite{tarvainen2017mean} and SESS~\cite{zhao2020sess}, we adopt an EMA teacher.
We further leverage asymmetric data augmentation and pseudo-label filtering (see Sec.\ref{sec:pseudo-label}).

To be in a position of advantage, the teacher network takes input data with weak augmentation only while the student network uses stronger data augmentation. 
We share the same data augmentation strategy with SESS. The input point clouds to our teacher network are augmented only by random sub-sampling while the inputs to the student network further undergo a set of stochastic transformation $\mathcal{T}$, including random flip, random rotation around the upright axis, and a random uniform scaling. 

% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}  

% \begin{table*}[h]
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
% & & \multicolumn{2}{c|}{5\%} & \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{20\%} & \multicolumn{2}{c|}{100\%} \\ 
%   \cline{3-10} \multirow{-2}{*}{Dataset} & \multirow{-2}{*}{Model} & \tabincell{c}{mAP\\@0.25} & \tabincell{c}{mAP\\@0.5} & \tabincell{c}{mAP\\@0.25} & \tabincell{c}{mAP\\@0.5} & \tabincell{c}{mAP\\@0.25} & \tabincell{c}{mAP\\@0.5} & \tabincell{c}{mAP\\@0.25} & \tabincell{c}{mAP\\@0.5} \\ \hline

% \multirow{5}{*}{ScanNet} & VoteNet  & 27.9±0.5 & 10.8±0.6 & 36.9±1.6 & 18.2±1.0 & 46.9±1.9 & 27.5±1.2 & 57.8 & 36.0 \\ \cline{2-10} 
% & SESS reported     & $\backslash$ & $\backslash$ & 39.7±0.9 & 18.6 & 47.9±0.4 & 26.9 & 62.1 & 38.8  \\ \cline{2-10} 
%                          & SESS     & 32.0±0.7 & 14.4±0.7 & 39.5±1.8 & 19.8±1.3 & 49.6±1.1 & 29.0±1.0 & 61.3 & 39.0  \\ \cline{2-10} 
%                          & Ours & \textbf{40.0±0.9} & \textbf{22.5±0.5} & \textbf{47.2±0.4} & \textbf{28.3±1.5} & \textbf{52.8±1.2} & \textbf{35.2±1.1} & \textbf{62.9} & \textbf{42.1} \\ \cline{2-10} 
%                          & Abs. improve. & +8.0 & +8.1 & +7.7 & +8.5 & +3.2 & +6.2 & +1.6 & +3.1 \\ \hline
% \multirow{5}{*}{SUN-RGBD} & VoteNet   & 29.9±1.5 & 10.5±0.5 & 38.9±0.8 & 17.2±1.3 & 45.7±0.6 & 22.5±0.8 & 58.0 & 33.4      \\ \cline{2-10} 
% & SESS reported     & $\backslash$ & $\backslash$ & 42.9±1.0 & 14.4 & 47.9±0.5 & 20.6 & 61.1 & 37.3  \\ \cline{2-10}
%                          & SESS      & 34.2±2.0 & 13.1±1.0 & 42.1±1.1 & 20.9±0.3 & 47.1±0.7 & 24.5±1.2 & 60.5 & 38.1  \\ \cline{2-10} 
%                          & Ours & \textbf{39.0±1.9} & \textbf{21.1±1.7} & \textbf{45.5±1.5} & \textbf{28.8±0.7} & \textbf{49.7±0.4} & \textbf{30.9±0.2} & \textbf{61.5} & \textbf{41.3} \\ \cline{2-10} 
%                          & Abs. improve. & +4.8 & +8.0 & +3.4 & +7.9 & +2.6 & +6.4 & +1.0 & +3.2  \\ \hline

% \end{tabular}
% \vspace{1mm}

% \caption{Comparison with VoteNet and SESS on ScanNet val set and SUN RGB-D val set under different ratios of labeled data. We report the mAP@0.25 and mAP@0.5 as mean±standard deviation across 3 runs under different random data splits. Due to the randomness of the data splits and our better pre-training protocol, SESS results provided by us are higher than those reported in the paper on mAP@0.5, and the mAP@0.25 results differ a little (the only difference is the pre-trained weights and data splits). The final improvement is the absolute improvement of our method over SESS results provided by us. Following SESS, we also report the results with 100\% labeled data, where we simply make a copy of the full dataset as unlabeled data and train our method.}
% \label{tab:main}
% \end{table*}

\subsection{Pseudo-Label Filtering and Deduplication}\label{sec:pseudo-label}
In the teacher-student framework, the performance gap between the teacher and the student is usually quite marginal given that these two models are just different by EMA on weight and data augmentation strength. Hence, it is not always true that the teacher prediction is more accurate than the student's on a specific training sample. On unlabeled data, the student model will only benefit from the pseudo-labels that are more accurate than its predictions. Therefore we should filter out low-quality predictions from the teacher model and only supervise the student model with the rest of the teacher model predictions.

%For image classification task, FixMatch\cite{sohn2020fixmatch} propose to use a classification confidence $\text{conf}_{cls} = \max\{p_{cls}\}$ defined as the top-1 probability in the predicted class distribution. FixMatch sets a confidence threshold $\tau_{cls}$ and only if $\text{conf}_{cls} > \tau_{cls}$ the pseudo-label will be kept. For 2D object detection, STAC\cite{sohn2020simple} first run NMS to remove duplicated bounding box predictions and then similarly leverages \yezhen{to fill} confidence for filtering.

%For two-stage detectors, e.g. Faster RCNN, region proposal network (RPN) will predict a confidence, which shares the same meaning of objectness score in VoteNet, for each region proposal and drop the ones with a confidence below 0.5\yezhen{No, this is different between test time and train time, which is complicated and subtle so I think maybe omitted (keep a fixed number of proposals instead of filtering)}. 
\mypara{Jointly filtering based on class, objectness, localization confidences}
For VoteNet, we propose to set an objectness threshold $\tau_{obj}$ and filter out bounding box predictions with objectness score $s < \tau_{obj}$. We further propose to set a classification confidence threshold $\tau_{cls}$ for filtering out predictions that are likely to contain a wrong class label. 

% However, for our 3D object detection task, it is not so straightforward to adopt confidence-based filtering. Compared to networks for image classification that only needs to predict one class probability distribution for an input data, VoteNet predicts multiple outputs for each bounding box $B_k$, including an object center position $\mathbf{c}$, a 3D bounding box size $\mathbf{d}$, an orientation angle $\theta$, a class probability distribution $p_{cls}$, and an objectness score $s$. 
Note that none of these two confidence measures capture the accuracy of bounding box parameter predictions. We propose to predict a 3D IoU for each predicted bounding box, use the 3D IoU estimation as a localization confidence, and set a localization threshold $\tau_\text{IoU}$ to filter out poorly localized predictions. Formally, we remove all the predictions that fail to satisfy all three confidence thresholds, i.e. $s > \tau_{obj}$, $\max(p_{cls}) > \tau_{cls}$, and $v > \tau_\text{IoU}$. 

\mypara{IoU-guided lower-half suppression for deduplication}
After the confidence-based filtering, there is still a lot of duplicated bounding box predictions that may introduce harmful noise to our pseudo-labels. NMS is a standard process in object detection for duplicate removal before evaluation, which takes a set of highly overlapped bounding box predictions that share the same class prediction, ranks them according to a confidence score and removes all but the top-1 prediction. STAC~\cite{sohn2020simple} applies class confidence based NMS to teacher predictions during pseudo-label generation. 

The default NMS used in VoteNet is based on objectness confidence. Given that objectness score doesn't capture the localization quality, a train-time IoU-guided NMS will naturally perform better (see Table.\ref{tab:ablation}), where we use the product of predicted IoU and predicted objectness as the ranking metric.
However, using the top one selected by IoU-guided NMS can still be suboptimal, since the predicted IoU will inevitably carry some errors. We argue that different from the test time scenario, pseudo-labels do not need to be fully deduplicated. Imagine this situation: if a  bounding box predicted by the student is $0.2 m$ to the left of its corresponding ground truth, it is a foreground object and will get bounding box supervision in VoteNet. However, if unfortunately the pseudo-label survives after non-maximal suppression is to the right of the ground truth more than $0.1m$, this predicted bounding box may lose supervision and be treated as a background box. This example shows that strict non-maximal suppression can lead to a smaller number of student model predictions that can receive supervision. Since we cannot know the best pseudo label among a bunch of highly-overlapped ones, it's fine to be less strict. To this end, we propose a novel Lower-Half Suppression, or in short, LHS, that only discards half of the proposals with lower predicted IoU.  We argue that since LHS suppresses bounding boxes sharing the same class label, this suppression can be seen as a second-step class-aware self-adjusted filtering, which sets dynamic thresholds among the overlapping bounding boxes to keep the ones with higher confidence and hence find a better balance between pseudo-label quality and the amount of supervision. We also use the product of predicted IoU and predicted objectness as the confidence metric.

%. In addition, this also means that more student model proposals gets supervised.

\mypara{Final-step pseudo-label processing}
After the filtering and IoU-guided LHS, we now have high-quality predictions $\{\hat{{y}}_T^u\}_{k=1}^{K'}$ from the teacher network, where $K'$ is the number of bounding boxes remains. Given that the student model inputs go through a stronger augmentation including an additional geometric transformation $\mathcal{T}$, in synchronize with the student model inputs, the bounding box parameters of the pseudo-labels need to go through the same transformation $\mathcal{T}$, namely $\tilde{{\boldsymbol b}}^u = \mathcal{T}(\hat{{\boldsymbol b}}_T^u)$. We further take convert the predicted class probability distribution $\hat{p}_T^u$ into semantic class label via $\tilde{q}^u = \max(\hat{p}_T^u)$. Now we obtain the filtered pseudo-labels $\tilde{y} = \{\tilde{\boldsymbol{b}}^u, \tilde{q}^u\}_{k=1}^{K'}$.

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}  

\begin{table*}[h]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
& & \multicolumn{2}{c|}{5\%} & \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{20\%} & \multicolumn{2}{c|}{100\%} \\ 
  \cline{3-10} \multirow{-2}{*}{Dataset} & \multirow{-2}{*}{Model} & \tabincell{c}{mAP\\@0.25} & \tabincell{c}{mAP\\@0.5} & \tabincell{c}{mAP\\@0.25} & \tabincell{c}{mAP\\@0.5} & \tabincell{c}{mAP\\@0.25} & \tabincell{c}{mAP\\@0.5} & \tabincell{c}{mAP\\@0.25} & \tabincell{c}{mAP\\@0.5} \\ \hline

\multirow{5}{*}{ScanNet} & VoteNet  & 27.9±0.5 & 10.8±0.6 & 36.9±1.6 & 18.2±1.0 & 46.9±1.9 & 27.5±1.2 & 57.8 & 36.0 \\ \cline{2-10} 
& SESS reported     & $\backslash$ & $\backslash$ & 39.7±0.9 & 18.6 & 47.9±0.4 & 26.9 & 62.1 & 38.8  \\ \cline{2-10} 
                         & SESS     & 32.0±0.7 & 14.4±0.7 & 39.5±1.8 & 19.8±1.3 & 49.6±1.1 & 29.0±1.0 & 61.3 & 39.0  \\ \cline{2-10} 
                         & Ours & \textbf{40.0±0.9} & \textbf{22.5±0.5} & \textbf{47.2±0.4} & \textbf{28.3±1.5} & \textbf{52.8±1.2} & \textbf{35.2±1.1} & \textbf{62.9} & \textbf{42.1} \\ \cline{2-10} 
                         & Abs. improve. & +8.0 & +8.1 & +7.7 & +8.5 & +3.2 & +6.2 & +1.6 & +3.1 \\ \hline
\multirow{5}{*}{SUN-RGBD} & VoteNet   & 29.9±1.5 & 10.5±0.5 & 38.9±0.8 & 17.2±1.3 & 45.7±0.6 & 22.5±0.8 & 58.0 & 33.4      \\ \cline{2-10} 
& SESS reported     & $\backslash$ & $\backslash$ & 42.9±1.0 & 14.4 & 47.9±0.5 & 20.6 & 61.1 & 37.3  \\ \cline{2-10}
                         & SESS      & 34.2±2.0 & 13.1±1.0 & 42.1±1.1 & 20.9±0.3 & 47.1±0.7 & 24.5±1.2 & 60.5 & 38.1  \\ \cline{2-10} 
                         & Ours & \textbf{39.0±1.9} & \textbf{21.1±1.7} & \textbf{45.5±1.5} & \textbf{28.8±0.7} & \textbf{49.7±0.4} & \textbf{30.9±0.2} & \textbf{61.5} & \textbf{41.3} \\ \cline{2-10} 
                         & Abs. improve. & +4.8 & +8.0 & +3.4 & +7.9 & +2.6 & +6.4 & +1.0 & +3.2  \\ \hline

\end{tabular}
\vspace{1mm}

\caption{Comparison with VoteNet and SESS on ScanNet val set and SUN RGB-D val set under different ratios of labeled data. We report the mAP@0.25 and mAP@0.5 as mean±standard deviation across 3 runs under different random data splits. Due to the randomness of the data splits and our better pre-training protocol, SESS results provided by us are higher than those reported in the paper on mAP@0.5, and the mAP@0.25 results differ a little (the only difference is the pre-trained weights and data splits). The final improvement is the absolute improvement of our method over SESS results provided by us. Following SESS, we also report the results with 100\% labeled data, where we simply make a copy of the full dataset as unlabeled data and train our method.}
\label{tab:main}
\end{table*}

\subsection{Selective Supervision using Pseudo-Labels}\label{sec:supervise}
%On unlabeled data, the student network takes pseudo-labels generated by the teacher model and filtered based on the three confidence scores. 
% For ground truth labels from labeled data, there are exactly $N = |O|$ bounding boxes. 


For our generated pseudo-labels, there is no guarantee that the labels can cover all the ground truth objects from $O$ due to the filtering and potentially inaccurate teacher predictions. Given the incompleteness of our filtered pseudo-labels, we are relatively confident about the bounding boxes in this set but student predictions far away from all of our pseudo-labels are not necessarily negative. Our experiments show that supervising objectness on unlabeled data using the pseudo-labels seriously hurts the performance. For similar reasons, we do not supervise vote loss, which is a unique element in VoteNet and not shown in other detectors. For more analysis and experimental proof for this, we refer the readers to the supplementary materials. 
In this case, we will only supervise the bounding boxes in the vicinity of the pseudo bounding boxes and aim to improve their bounding box quality. More specifically, we stick to the way how VoteNet select foreground objects for bounding box parameter supervision: we supervise bounding box parameters and class for a prediction only if the vote that generates this prediction is within $0.3 \text{m}$ of any bounding box in the pseudo-labels. For this set of pseudo-foreground predictions, we adopt the same way that VoteNet establishes association and enforce original VoteNet losses except for objectness loss and vote loss.




==> [CVPR 21] 3DIoUMatch/tex/04_experiment.tex <==





% \begin{table*}[h]
% \begin{tabular}{c|c|c|cccc}
% \hline
% Dataset                  & Model                       & Metric      & 5\% & 10\% & 20\% & 100\% \\ \hline
% \multirow{8}{*}{ScanNet} & \multirow{2}{*}{VoteNet}    & mAP@0.25 & 27.92 (±0.51) & 36.93 (±1.61) & 46.88 (±1.92) & 58.50      \\ \cline{3-7} 
%                          &                             & mAP@0.5  & 10.81 (±0.60) & 18.20 (±0.96) & 27.47 (±1.23) & 36.24      \\ \cline{2-7} 
%                          & \multirow{2}{*}{SESS}       & mAP@0.25 & 31.96 (±0.72) & 39.54 (±1.78) & 49.57 (±1.06) & 62.10      \\ \cline{3-7} 
%                          &                             & mAP@0.5  & 14.43 (±0.70) & 19.84 (±1.35) & 28.98 (±0.97) & 38.80      \\ \cline{2-7} 
%                          & \multirow{2}{*}{FixMatch}   & mAP@0.25 & 35.87 (±1.44) & 44.48 (±1.54) & 51.66 (±0.96) & 61.62      \\ \cline{3-7} 
%                          &                             & mAP@0.5  & 18.36 (±0.71) & 24.65 (±1.61) & 32.34 (±0.35) & 39.33      \\ \cline{2-7} 
%                          & \multirow{2}{*}{3DIoUMatch} & mAP@0.25 & \textbf{40.00 (±0.92)} & \textbf{47.15 (±0.40)} & \textbf{52.82 (±1.17)} & \textbf{62.93}      \\ \cline{3-7} 
%                          &                            & mAP@0.5  & \textbf{22.53 (±0.50)} & \textbf{28.33 (±1.55)} & \textbf{35.19 (±1.06)} & \textbf{42.10}       \\ \hline
% \multirow{8}{*}{SUN-RGBD} & \multirow{2}{*}{VoteNet}    & mAP@0.25 & 29.93 (±1.52) & 38.89 (±0.78) & 45.66 (±0.61) &       \\ \cline{3-7} 
%                          &                             & mAP@0.5  & 10.53 (±0.48) & 17.20 (±1.31) & 22.47 (±0.85) &       \\ \cline{2-7} 
%                          & \multirow{2}{*}{SESS}       & mAP@0.25 & 34.16 (±1.99) & 42.08 (±1.11) & 47.04 (±0.70) &       \\ \cline{3-7} 
%                          &                             & mAP@0.5  & 13.11 (±1.04) & 20.90 (±0.29) & 24.47 (±1.20) &       \\ \cline{2-7} 
%                          & \multirow{2}{*}{FixMatch}   & mAP@0.25 & 36.87 (±2.38) & 42.92 (±1.05) & 47.45 (±0.69) & 60.19      \\ \cline{3-7} 
%                          &                             & mAP@0.5  & 17.50 (±1.68) & 24.37 (±0.78) & 26.10 (±0.82) & 37.15      \\ \cline{2-7} 
%                          & \multirow{2}{*}{3DIoUMatch} & mAP@0.25 & \textbf{39.02 (±1.93)} & \textbf{45.53 (±1.48)} & \textbf{49.29 (±0.80)}     & \textbf{61.34}      \\ \cline{3-7} 
%                          &                             & mAP@0.5  & \textbf{21.05 (±1.72)} & \textbf{28.82 (±0.67)} & \textbf{30.77 (±0.11)}     & \textbf{40.07}      \\ \hline

% \end{tabular}
% \caption{result}
% \end{table*}

\subsection{Datasets and Evaluation Metrics}

\paragraph{Indoor Datasets: ScanNet and SUNRGB-D}
We evaluate our VoteNet-based 3DIoUMatch on two major indoor datasets, ScanNet~\cite{dai2017scannet} and SUN RGB-D~\cite{song2015sun}. ScanNet is an indoor scene dataset consisting of 1513 reconstructed meshes, among which 1201 are training samples and the rest are validation samples. SUN RGB-D contains 10335 RGB-D images of indoor scenes which are split into 5285 training samples and 5050 validation samples. For both datasets, we follow~\cite{qi2019deep,zhao2020sess} for pre-processing data and labels to train our method and we report mAP@0.25 (mean average precision with 3D IoU threshold 0.25) and mAP@0.5 in the following experiments.

\paragraph{Outdoor Dataset: KITTI}
As for our PV-RCNN-based 3DIoUMatch, we use KITTI for evaluation. KITTI \cite{geiger2013vision} is a very popular dataset for autonomous driving which consists of fine annotations for 3D detection. There are 7481 outdoor scenes for training and 7518 for testing, and the training samples are generally divided into a train split of 3712 samples and a validation split of 3769 samples. We follow~\cite{shi2020pv} for data pre-processing and report the mAP with 40 recall positions, with a rotated IoU threshold 0.7, 0.5, 0.5 for the three classes, car, pedestrian, and cyclist, respectively.


\begin{table*}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
 & & & & & \multicolumn{2}{c|}{ScanNet 10\%} & \multicolumn{2}{c|}{SUN-RGBD 5\%} \\ 
 \cline{6-9} \multirow{-2}{*}{\tabincell{c}{Obj\&Cls\\Filter}} &  
  \multirow{-2}{*}{\tabincell{c}{IoU\\Filter}} &
 \multirow{-2}{*}{\tabincell{c}{Train-time\\Suppression}} & 
 \multirow{-2}{*}{\tabincell{c}{Test-time\\Suppression}} & 
 \multirow{-2}{*}{\tabincell{c}{Test-time\\IoU opt.}} & 
 mAP@0.25 & mAP@0.5 & mAP@0.25  & mAP@0.5 \\ \hline
 & & & Obj-NMS & & 38.4 & 19.8 & 32.9 & 12.5 \\ \hline
\checkmark & & & Obj-NMS & & 44.5 & 24.7 & 36.9 & 17.5 \\ \hline
%\checkmark & \checkmark & & Obj-NMS & & 44.9 & 25.3 & 37.3 & 17.7 \\ \hline
\checkmark & & Obj-NMS & Obj-NMS & & 44.2 & 25.2 & 37.1 & 17.4 \\ \hline \hline
\checkmark & \checkmark & IoU-NMS & Obj-NMS & & 45.9 & 26.8 & 37.4 & 18.7 \\ \hline
% \checkmark &  \checkmark & IoU-NMS & IoU-NMS & & 46.4 & 28.2 & 38.0 & 20.9 \\ \hline 
% \checkmark & \checkmark & IoU-NMS & IoU-NMS & \checkmark & 46.5 & \textbf{28.3} & 38.2 & \textbf{21.1} \\ \hline 
\checkmark & \checkmark & IoU-LHS & Obj-NMS & & 46.5 & 26.9 & 37.9 & 18.5 \\ \hline
\checkmark &  \checkmark & IoU-LHS & IoU-NMS & & 47.0 & 28.2 & 38.8 & 20.8 \\ \hline

\checkmark & \checkmark & IoU-LHS & IoU-NMS & \checkmark & \textbf{47.2} & \textbf{28.3} & \textbf{39.0} & \textbf{21.1} \\ \hline
\end{tabular}
\vspace{1mm}
\caption{Effects of the different components, including train-time filtering and deduplication, and test-time improvements.}
\label{tab:ablation}
\end{table*}

\subsection{Experiments on Indoor Scene Datasets}
%\subsection{Implementation Details}
For experiments on indoor datasets, \textit{i.e.}, ScanNet and SUNRGB-D, we use IoU-aware VoteNet as our backbone detector.

\subsubsection{Result Comparison}

Table \ref{tab:main} shows the results of our method compared to SESS and VoteNet under different ratios of labeled data on ScanNet and SUN RGB-D, respectively. The results illustrate that, with our effective train-time filtering and test-time improvement leveraging IoU estimation, we are able to significantly outperform current state-of-the-art, SESS, under all labeled ratio settings. With 5\% labeled
data, our method outperforms SESS by \textbf{8.1} and \textbf{8.0} on mAP@0.5 on ScanNet and SUN RGB-D, respectively. Note that our method gains more improvement on mAP@0.5, thanks to the high quality of pseudo labels and the IoU guidance for test-time NMS. 

% From the per-class performance on ScanNet in Table \ref{tab:scanperclass1}, we can see that our method outperforms SESS in almost every class, and leveraging IoU brings considerable improvement in most classes.

\subsubsection{Ablation Study}
\paragraph{Filtering and Deduplication Mechanism.}
We study the effect of each component of the filtering and deduplication mechanism. In Table \ref{tab:ablation}, the second row shows the results of naive pseudo labeling, which takes all predictions from the teacher model for supervision. Expectedly the results are not satisfying, only a little higher than VoteNet. Simply applying the dual filtering of classification and objectness confidence gives significant improvement, as the filtering picks out the teacher model proposals that are very likely to be close to true objects and have the correct class. The conventional objectness-based NMS in VoteNet, however, fails to improve further, since the remaining proposals already have high objectness scores and the objectness-based NMS is not capable of picking the ones with higher localization accuracy.

As shown in the fifth and sixth row, after we introduce IoU during train time, IoU filtering and train-time IoU-guided NMS contribute to better performance under both settings. Our proposed IoU-guided LHS improves over IoU guided NMS on mAP@0.25, since LHS finds a better balance between quality and coverage. With better filtering and deduplication leveraging IoU estimation during train time, we gain 2.3 and 1.7 absolute improvement over the without-IoU version on mAP@0.25 and mAP@0.5 respectively on ScanNet 10\%. This verifies that considering localization confidence is important for getting high-quality pseudo labels. With test-time improvements, our method gains in total 3.0 and 3.1 absolute improvement respectively.

We set 0.9 for both classification and objectness confidence threshold following STAC~\cite{sohn2020simple} and investigate the effect of different IoU thresholds on ScanNet 10\%, as shown in Figure \ref{fig:iou}. The performance (with test-time improvements) is higher than the without-IoU baseline by large margins when $\tau_{IoU} \leq 0.5$. Note that the performance peaks at $\tau_{IoU} = 0.25$ for mAP@0.25 while peaking at 0.5 for mAP@0.5, simply because mAP@0.5 prefers a stronger filtering on localization quality. When $\tau_{IoU} > 0.5$ , further increasing  $\tau_{IoU}$ may lead to a drastic drop in pseudo-label coverage and hence is detrimental to the performance.
%Intuitively, setting the value of the IoU threshold is a balance between higher quality and more supervision, and though the IoU estimation has some error, it still qualifies as a good filtering metric.

\paragraph{Test-time IoU-guided NMS and IoU optimization.}
We then evaluate the improvement brought by using IoU estimations at test time. The last two rows in Table \ref{tab:ablation} shows that IoU-guided NMS and IoU optimization improves the performance further.


\subsubsection{Result Analysis}
In this section, we examine how our 3DIoUMatch works during training on ScanNet 10\%. The upper two curves in Figure \ref{fig:stats} show that as the training goes, the performance on unlabeled data and test data increases conformably, which indicates the increasing quality of pseudo-labels. We also show how the coverage of the pseudo-labels changes on the unlabeled data over the training. Here coverage at a certain threshold simply means the class-agnostic recall, measuring the percentage of ground truth objects that can find a pseudo-label with an IoU larger than the threshold.
As we can see from the lower two curves in Figure \ref{fig:stats}: at the beginning, the coverage of the pseudo-labels is relatively low due to the strict filtering mechanism; as the semi-supervised learning goes on, the improving detection performance leads to a higher passing rate of the filter and hence a higher coverage of the pseudo-labels, which in return fuels SSL; by the end of training, the coverage at 0.25 and at 0.5 both increase by about 10\%. 

\begin{figure}[t]
\begin{center}
   \includegraphics[width=1.0\linewidth]{figure/curve-iou.pdf}
\end{center}
   \caption{3DIoUMatch results with different IoU thresholds on ScanNet 10\%.}
\label{fig:long}
\label{fig:onecol}
\label{fig:iou}
\end{figure}

\begin{figure}[t]
\begin{center}
   \includegraphics[width=1.0\linewidth]{figure/curve-statistics.pdf}
\end{center}
   \caption{The performance improvements and pseudo-label coverage over the semi-supervised learning stage on ScanNet 10\%.}
\label{fig:long}
\label{fig:onecol}
\label{fig:stats}
\end{figure}

% \begin{table*}[t]
% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{ccccccccccccccccccc}
% \hline
% & \multicolumn{1}{l}{cab} & \multicolumn{1}{l}{bed} & \multicolumn{1}{l}{chair} & \multicolumn{1}{l}{sofa} & \multicolumn{1}{l}{table} & \multicolumn{1}{l}{door} & \multicolumn{1}{l}{wind} & \multicolumn{1}{l}{bkshf} & \multicolumn{1}{l}{pic} & \multicolumn{1}{l}{cntr} & \multicolumn{1}{l}{desk} & \multicolumn{1}{l}{curt} & \multicolumn{1}{l}{fridg} & \multicolumn{1}{l}{showr} & \multicolumn{1}{l}{toil} & \multicolumn{1}{l}{sink} & \multicolumn{1}{l}{bath} & \multicolumn{1}{l}{ofurn} \\ \hline\hline
% VoteNet mAP@0.25     & 17.9                        & 74.7                    & 74.5                      & 75.3                     & 45.6                      & 18.3                     & 11.7                       & 21.7                          & 0.7                         & 28.4                        & 49.4                     & 21.5                        & 23.2                             & 18.5                               & 79.6                       & 25.7                     & 66.3                        & 11.7                           \\ \hline

% SESS mAP@0.25        & 20.5                        & 75.1                    & 76.2                      & 76.4                     & 48.1                      & 20.0                     & 14.4                       & 19.4                          & 1.2                         & 30.0                        & 51.8                     & 25.0                        & 30.0                             & 26.4                               & 82.2                       & 29.2                     & 72.3                        & 14.1                           \\ \hline

% Without IoU mAP@0.25 & 22.6                        & 79.5                    & 77.8                      & 77.8                     & 49.6                      & 25.4                     & 18.6                       & 27.7                          & 3.3                         & 41.4                        & 56.2                     & 27.4                        & 30.4                             & \textbf{53.6}                      & 81.3                       & 28.5                     & 74.5                        & 18.8                           \\ \hline

% 3DIoUMatch mAP@0.25  & \textbf{26.6}               & \textbf{82.6}           & \textbf{80.9}             & \textbf{83.3}            & \textbf{52.1}             & \textbf{28.0}            & \textbf{19.9}              & \textbf{29.4}                 & \textbf{3.7}                & \textbf{45.0}               & \textbf{61.9}            & \textbf{29.2}               & \textbf{34.1}                    & 51.2                               & \textbf{85.7}              & \textbf{32.3}            & \textbf{82.8}               & \textbf{21.5}                  \\ \hline\hline
% VoteNet mAP@0.5      & 3.2                         & 64.6                    & 43.4                      & 49.3                     & 25.1                      & 2.8                      & 1.1                        & 8.7                           & 0.0                         & 2.4                         & 14.7                     & 3.9                         & 7.6                              & 1.1                                & 46.8                       & 11.9                     & 39.4                        & 1.5                            \\ \hline
% SESS mAP@0.5         & 3.7                         & 61.2                    & 48.0                      & 44.8                     & 29.5                      & 3.2                      & 2.8                        & 8.4                           & 0.2                         & 7.5                         & 19.2                     & 5.0                         & 12.2                             & 1.8                                & 48.7                       & \textbf{15.3}            & 40.8                        & 2.2                            \\ \hline
% Without IoU mAP@0.5  & 3.9                         & 66.1                    & 52.7                      & 50.7                     & 35.1                      & 7.9                      & 5.0                        & 13.1                          & \textbf{0.9}                & 14.5                        & 26.1                     & \textbf{10.3}               & 17.5                             & \textbf{7.0}                       & 63.9                       & 11.7                     & 62.1                        & 4.9                            \\ \hline
% 3DIoUMatch mAP@0.5   & \textbf{5.9}                & \textbf{72.0}           & \textbf{60.5}             & \textbf{56.6}            & \textbf{39.7}             & \textbf{10.3}            & \textbf{5.2}               & \textbf{18.1}                 & 0.7                         & \textbf{16.0}               & \textbf{35.3}            & 8.3                         & \textbf{21.4}                    & 6.2                                & \textbf{67.5}              & 13.2                     & \textbf{67.6}               & \textbf{5.2}                   \\ \hline
% \end{tabular}
% \end{adjustbox}
% \vspace{1mm}
% \caption{Per class mAP@0.25 and mAP@0.5 on ScanNet val set, with 10\% labeled data. The bold numbers are the highest per class.}
% \label{tab:scanperclass1}
% \end{table*}


%\yezhen{The following implementation details are for VoteNet-based 3DIoUMatch. For the PV-RCNN-based counterpart, please refer to \ref{sec:kitti}.}
\subsubsection{Implementation Details}
\mypara{Training}
% We feed training batches of point clouds with 5,000 points to our framework. To construct a batch, we randomly sample Bl labeled samples from PL
% and Bu unlabeled samples from PU. In the experiments,
% Bl is set to 2 and Bu to 8. During the perturbation step, the
% number of randomly sub-sampled points is 4,000; the ϑ is
% set to 30◦ on SUN RGB-D and 5◦ on ScanNetV2; the random
% scale range is bounded by a = 0.85 and b = 1.15. The
% weights in the consistency loss function are set as λ1 = 1,
% λ1 = 2, λ3 = 1. As suggested in [22], we ramp up the
% coefficient of consistency cost from 0 to its maximum value
% of 10 during the first 30 epochs, using a sigmoid-shaped
% function e−5(1−T)2
% , where T increases linearly from 0 to 1
% during the ramp-up period. In terms of EMA decay α, we
% set α = 0.99 during the ramp-up period, and α = 0.999 for
% the rest of the training, following
For the pre-training stage, we train with a batch size of 8 and follow the same data augmentation of SESS~\cite{zhao2020sess}.  We then use those pre-trained weights to initialize the student and teacher networks. 
For the SSL stage, we construct each batch by taking 4 labeled samples and 8 unlabeled samples, with the same data augmentation. The weights of different loss terms are the same as VoteNet and we set $\lambda_{u}=2$. The student network is trained for 1000 epochs (the labeled data is traversed in one epoch), optimized by an ADAM optimizer with an initial learning rate of 0.002, and the learning rate is decayed
by 0.3, 0.3, 0.1, 0.1 at the 400\textsuperscript{th}, 600\textsuperscript{th}, 800\textsuperscript{th} and 900\textsuperscript{th} epoch, respectively. The number of generated 3D proposals is 128. We use $k=3, D=4$ for the IoU module. The three thresholds are set to be $\tau_{obj}=0.9, \tau_{cls}=0.9, \tau_{IoU}=0.25$. 
% To train the IoU estimation branch in both stages, following IoU-Net\cite{jiang2018acquisition}, we jitter the bounding box predictions by adding Gaussian noise to the box center and size to create 128 more training samples of IoU estimation for each scene. We use L1 loss for IoU estimation loss. 
For more details, we refer the readers to the supplementary materials.
% In stage 2, we only supervise IoU on the labeled part.

\mypara{Inference}
We forward the input to the student network to generate proposals. We first apply IoU optimization to refine box parameters following IoU-Net~\cite{jiang2018acquisition}, followed by an IoU-guided NMS with a 3D IoU threshold of 0.25.
% (THIS WAS MENTIONED BEFORE) and the score for each bounding box is the product of IoU estimation and objectness score, instead of IoU estimation alone as used in IoU-Net. 
% Following \cite{qi2019deep, zhao2020sess}, we report mAP@0.25 (mean average precision with 3D IoU threshold 0.25) and mAP@0.5 in the following experiments.


% \begin{figure*}[t]
% \begin{center}
%   \includegraphics[width=0.8\linewidth]{figure/placeholder.png}
% \end{center}
%   \caption{placeholder.}
% \label{fig:long}
% \end{figure*}





\subsection{Experiments on KITTI}\label{sec:kitti}
For experiments on the KITTI dataset,  we adopt PV-RCNN\cite{shi2020pv} as our backbone\footnote{Update to the CVPR camera-ready version: to avoid information leakage, we no longer apply the ground truth sampling augmentation used by PV-RCNN to unlabeled data in 1\% and 2\% labeled data experiments. We therefore retrain the networks and update the results in Table 3 and 4. See supplementary materials for more details.}. PV-RCNN itself comes with a 3D IoU module, allowing to use it in our semi-supervised learning pipeline without modifying its architecture.
% Different from ScanNet and SUNRGBD, which are indoor 3D datasets, KITTI is a large outdoor 3D dataset. To examine the generality of our method, we apply our method on the SOTA detector, PV-RCNN \cite{shi2020pv}. Here we do not use VoteNet because of its incapability to handle huge outdoor scenes.
% %We follow the same two-stage training scheme as done in our submission. 
% PV-RCNN itself contains an IoU confidence module directly enabling IoU filtering. On KITTI, it has different hyperparameters for the three classes.  We hence choose IoU threshold $\tau_{car}= 0.8$, $\tau_{ped}=\tau_{cyc} = 0.4$, and $\tau_{cls}=0.2$. We selectively supervise the predictions that meet foreground bar according to our pseudo-labels.
% %For selective supervision on unlabeled data, we only supervise the student's predictions with higher than 0.3 IoU with any pseudo-labels.
\vspace{-3mm}
\subsubsection{Results}
We evaluate our method on KITTI validation set. Table \ref{tab:kitti_main} demonstrates significant and consistent improvement across all categories with 1\%, 2\%, and 100\% labeled data, compared to supervised training only. Similar to our experiments on indoor scene datasets, here the 100\% labeled data setting means making a copy of the full dataset as unlabeled data and training the network using our devised semi-supervised pipeline. With 2\% labeled data, our method outperforms the labeled-data-only baseline by 7.4 and 10.7 mAP@0.5 on pedestrian and cyclist, respectively, which are very challenging for low data ratios.

\vspace{-3mm}
\subsubsection{Ablation Study}
We conduct ablation studies on KITTI with 1\% labeled data. Table \ref{tab:kitti_ablate} shows our improvements compared with a pseudo-label baseline and filtering based on class confidence only. The results validate the effectiveness of our IoU-based localization confidence filtering.

\vspace{-3mm}

\subsubsection{Implementation Differences with VoteNet}
% old version
% %Different from VoteNet, PV-RCNN itself contains an IoU confidence module, and we directly adopt this module for IoU filtering. 
% In KITTI, we only care about three classes, car, pedestrian, and cyclist, which differ a lot in the difficulty to detect. 
% Instead of using LHS, we follow PV-RCNN to set different IoU thresholds for each individual class, \textit{i.e.},
% %Therefore, we set different IoU thresholds for the three classes,
% $\tau_{car}= 0.8$, $\tau_{ped}=\tau_{cyc} = 0.4$. We selectively supervise the predictions that meet the foreground bar in PV-RCNN according to our pseudo-labels.
% In contrast to VoteNet, PV-RCNN is a two-stage detector containing an RPN. Bounding box objectness (or foreground probability) has been predicted in the RPN and used to pick top 100 proposals to forward to the RoI head. We therefore only additionally filter according to classification confidence with the threshold $\tau_{cls}=0.2$. 
%objectness, , is used in the RPN. Since the RPN itself already sets a threshold on objectness, we do not add another one for pseudo-label filtering. We only set a classification probability threshold $\tau_{cls}=0.2$.

% new version
In KITTI, we only care about three classes, car, pedestrian, and cyclist, which differ a lot in the difficulty to detect. 
Instead of using LHS, we follow PV-RCNN to set different IoU thresholds for each individual class, \textit{i.e.},
%Therefore, we set different IoU thresholds for the three classes,
$\tau_{car}= 0.5$, $\tau_{ped}=\tau_{cyc} = 0.25$. %We selectively supervise the predictions that meet the foreground bar in PV-RCNN according to our pseudo-labels.
In contrast to VoteNet, PV-RCNN is a two-stage detector containing an RPN. After the RPN stage, only a number of proposals are kept based on classification score, which acts like objectness score in VoteNet. We further filter with the classification score obtained from the RPN stage, with a threshold of $\tau_{cls}=0.4$.

Due to the non-differentiability of the IoU module of PV-RCNN, we do not apply IoU optimization.

We also adopt a two-stage training scheme for our PV-RCNN-based 3DIoUMatch. We use an unlabeled weight $\lambda_{u}=1$ and only supervise anchor classification and bounding box regression in PV-RCNN on unlabeled data. Please refer to the supplementary materials for more details.
%\footnote{The implementation details differ with the previous version of our paper due to a mistake. In the latest version, we fixed the mistake.}


% \subsection{Limitations}
% \verify{needs modification since this is VoteNet-specific}
% As discussed in \ref{sec:supervise}, we do not supervise objectness loss and vote loss on unlabeled data due to the uncertainty about negative samples. Also, we do not supervise the 3D IoU module on unlabeled data. We expect further performance improvements if the unlabeled data can be utilized to improve their training.

% \begin{table}[t]
%  \resizebox{\columnwidth}{!}{
%       \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%     & \multicolumn{3}{c|}{1\%} & \multicolumn{3}{c|}{2\%} & \multicolumn{3}{c|}{100\%}\\ 
%       \cline{2-10} \multirow{-2}{*}{} & Car & Ped. & Cyc. & Car & Ped. & Cyc. & Car & Ped. & Cyc.  \\ \hline
%     PVR. & 77.3 & 47.8 & 62.9 & 80.4 & 47.1 & 63.5 & 83.0 & 57.9 & 73.1 \\ \cline{1-10} 
%     Ours & \textbf{80.7} & \textbf{54.4} & \textbf{67.3} & \textbf{82.0} & \textbf{54.6} & \textbf{69.5} & \textbf{84.8} & \textbf{60.2} & \textbf{74.9} \\ \cline{1-10} 
%     Improvements & \t extbf{+3.4} & \textbf{+6.6} & \textbf{+4.4} & \textbf{+1.6} & \textbf{+7.5} & \textbf{+6.0} & \textbf{+1.8} & \textbf{+2.3} & \textbf{+1.8} \\ \cline{1-10} 
%     % $\tau_{obj}=\tau_{cls}=0.95$ & & & & & & \\ \cline{1-7} 
%     % $\lambda = 1$ & & & 37.5 & 21.0 & & \\ \cline{1-7}
%     % $\lambda = 4$ & & & 38.6 & 20.5 & & \\ \cline{1-7} 
%     % $k=5$ &  &  &  &  & & \\ \cline{1-7} 
%     \end{tabular}
%     }
% \vspace{1mm}
%     \caption{\textbf{3D detection results on KITTI val set with different labeled ratios.} The results are for moderate difficulty level evaluated by the mAP with 40 recall positions, with a rotated IoU threshold 0.7, 0.5, 0.5 for the three classes, respectively.}
%     \label{tab:kitti_main}
    
% \end{table}

% \begin{table}[t]
%  \resizebox{\columnwidth}{!}{
% %     \begin{minipage}{0.7\textwidth}
%       \centering
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
% & \multicolumn{3}{c|}{Car} & \multicolumn{3}{c|}{Pedestrian} & \multicolumn{3}{c|}{Cyclist}\\ 
%   \cline{2-10} \multirow{-2}{*}{} & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard  \\ \hline
% PVR. & 89.6 & 77.3& 74.1 & 54.9 & 47.8 & 42.3 & 80.4 & 62.9 & 58.7 \\ \cline{1-10} 
% naive psd.-lb. & 91.1 & 78.8 & 76.1 & 58.9 & 51.3 & 45.4 & 82.6 & 65.5 & 60.8 \\ \cline{1-10}
% cls. thres. only & 90.8 & 79.7 & 76.8 & 63.2 & \textbf{55.0} & \textbf{49.7} & 84.9 & 65.0 & 61.2 \\ \cline{1-10} 
% % $\tau_{obj}=\tau_{cls}=0.95$ & & & & & & \\ \cline{1-7} 
% % $\lambda = 1$ & & & 37.5 & 21.0 & & \\ \cline{1-7}
% % $\lambda = 4$ & & & 38.6 & 20.5 & & \\ \cline{1-7} 
% % $k=5$ &  &  &  &  & & \\ \cline{1-7} 
% Ours & \textbf{91.6} & \textbf{80.7} & \textbf{78.1} & \textbf{63.3} & 54.4 & 49.5 & \textbf{86.5} & \textbf{67.3} & \textbf{62.8} \\ \hline
% \end{tabular}
%     }
% \vspace{1mm}
% \caption{\textbf{Ablation study on KITTI 1\% labeled data. }Same evaluation metric as Table 1. %NPL: naive pseudo-label, Cls: only filtering based on class confidence. 
% }
% \label{tab:kitti_ablate}
% % \end{minipage}

% \end{table}

\begin{table}[t]
 \resizebox{\columnwidth}{!}{
      \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    & \multicolumn{3}{c|}{1\%} & \multicolumn{3}{c|}{2\%} & \multicolumn{3}{c|}{100\%}\\ 
      \cline{2-10} \multirow{-2}{*}{} & Car & Ped. & Cyc. & Car & Ped. & Cyc. & Car & Ped. & Cyc.  \\ \hline
    PVR. & 73.5 & 28.7 & 28.4 & 76.6 & 40.8 & 45.5 & 83.0 & 57.9 & 73.1 \\ \cline{1-10} 
    Ours & \textbf{76.0} & \textbf{31.7} & \textbf{36.4} & \textbf{78.7} & \textbf{48.2} & \textbf{56.2} & \textbf{84.8} & \textbf{60.2} & \textbf{74.9} \\ \cline{1-10} 
    Improvements & \textbf{+2.5} & \textbf{+3.0} & \textbf{+8.0} & \textbf{+2.1} & \textbf{+7.4} & \textbf{+10.7} & \textbf{+1.8} & \textbf{+2.3} & \textbf{+1.8} \\ \cline{1-10} 
    % $\tau_{obj}=\tau_{cls}=0.95$ & & & & & & \\ \cline{1-7} 
    % $\lambda = 1$ & & & 37.5 & 21.0 & & \\ \cline{1-7}
    % $\lambda = 4$ & & & 38.6 & 20.5 & & \\ \cline{1-7} 
    % $k=5$ &  &  &  &  & & \\ \cline{1-7} 
    \end{tabular}
    }
\vspace{1mm}
    \caption{\textbf{3D detection results on KITTI val set with different labeled ratios.} The results are for moderate difficulty level evaluated by the mAP with 40 recall positions, with a rotated IoU threshold 0.7, 0.5, 0.5 for the three classes, respectively.}
    \label{tab:kitti_main}
    
\end{table}


\begin{table}[t]
 \resizebox{\columnwidth}{!}{
%     \begin{minipage}{0.7\textwidth}
      \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
& \multicolumn{3}{c|}{Car} & \multicolumn{3}{c|}{Pedestrian} & \multicolumn{3}{c|}{Cyclist}\\ 
  \cline{2-10} \multirow{-2}{*}{} & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard  \\ \hline
PVR. & 87.7 & 73.5 & 67.7 & 32.4 & 28.7 & 26.2 & 48.1 & 28.4 & 27.1 \\ \cline{1-10} 
naive psd.-lb. & 88.4 & 75.2 & 69.5 & 32.7 & 29.2 & 26.7 & 51.4 & 30.7 & 28.7 \\ \cline{1-10}
cls. filt. only & 87.9 & 75.5 & 70.5 & 36.6 & 31.0 & 28.3 & 57.3 & 35.3 & 33.0 \\ \cline{1-10} 
% $\tau_{obj}=\tau_{cls}=0.95$ & & & & & & \\ \cline{1-7} 
% $\lambda = 1$ & & & 37.5 & 21.0 & & \\ \cline{1-7}
% $\lambda = 4$ & & & 38.6 & 20.5 & & \\ \cline{1-7} 
% $k=5$ &  &  &  &  & & \\ \cline{1-7} 
Ours & \textbf{89.0} & \textbf{76.0} & \textbf{70.8} & \textbf{37.0} & \textbf{31.7} & \textbf{29.1} & \textbf{60.4} & \textbf{36.4} & \textbf{34.3} \\ \hline
\end{tabular}
    }
\vspace{1mm}
\caption{\textbf{Ablation study on KITTI 1\% labeled data. }Same evaluation metric as Table 1. %NPL: naive pseudo-label, Cls: only filtering based on class confidence. 
}
\label{tab:kitti_ablate}
% \end{minipage}
\vspace{-2mm}

\end{table}





==> [CVPR 21] 3DIoUMatch/tex/05_conclusion.tex <==
In this paper, we propose 3DIoUMatch, a novel semi-supervised 3D object detection method leveraging IoU estimation. Built upon a teacher-student mutual learning framework, we leverage asymmetric data augmentation and pseudo-label filtering and deduplication to facilitate the student learning from the EMA teacher. With our IoU estimation module, we make filtering and deduplication aware of localization confidence and apply test-time IoU-guided NMS and IoU optimization, leading to further improvement. Experiment results on the ScanNet, SUN-RGBD, and KITTI datasets validate the effectiveness of our method: we achieve significant gain over the previous state-of-the-art methods and baselines under all settings. Our idea of leveraging IoU estimation for semi-supervised learning is generally applicable to different kinds of 3D object detectors and can be extended to 2D detectors as future works.


% I think we should split this into 0.25 & 0.5?
% \begin{table}[h]
% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{lllllllllllllllllll}
% \hline
%                   & \multicolumn{1}{l}{cab} & \multicolumn{1}{l}{bed} & \multicolumn{1}{l}{chair} & \multicolumn{1}{l}{sofa} & \multicolumn{1}{l}{table} & \multicolumn{1}{l}{door} & \multicolumn{1}{l}{wind} & \multicolumn{1}{l}{bkshf} & \multicolumn{1}{l}{pic} & \multicolumn{1}{l}{cntr} & \multicolumn{1}{l}{desk} & \multicolumn{1}{l}{curt} & \multicolumn{1}{l}{fridg} & \multicolumn{1}{l}{showr} & \multicolumn{1}{l}{toil} & \multicolumn{1}{l}{sink} & \multicolumn{1}{l}{bath} & \multicolumn{1}{l}{ofurn} \\ \hline
% VoteNet mAP@0.25  & 0.179                       & 0.747                   & 0.745                     & 0.753                    & 0.456                     & 0.183                    & 0.117                      & 0.217                         & 0.007                       & 0.284                       & 0.494                    & 0.215                       & 0.232                            & 0.185                              & 0.796                      & 0.257                    & 0.663                       & 0.117                          \\
% VoteNet mAP@0.5   & 0.032                       & 0.646                   & 0.434                     & 0.493                    & 0.251                     & 0.028                    & 0.011                      & 0.087                         & 0                           & 0.024                       & 0.147                    & 0.039                       & 0.076                            & 0.011                              & 0.468                      & 0.119                    & 0.394                       & 0.015                          \\
% SESS mAP@0.25     & 0.205                       & 0.751                   & 0.762                     & 0.764                    & 0.481                     & 0.2                      & 0.144                      & 0.194                         & 0.012                       & 0.3                         & 0.518                    & 0.25                        & 0.3                              & 0.264                              & 0.822                      & 0.292                    & 0.723                       & 0.141                          \\
% SESS mAP@0.5      & 0.037                       & 0.612                   & 0.48                      & 0.448                    & 0.295                     & 0.032                    & 0.028                      & 0.084                         & 0.002                       & 0.075                       & 0.192                    & 0.05                        & 0.122                            & 0.018                              & 0.487                      & \textbf{0.153}           & 0.408                       & 0.022                          \\ \hline \hline
% IoUMatch mAP@0.25 & \textbf{0.264}              & \textbf{0.826}          & \textbf{0.809}            & \textbf{0.832}           & \textbf{0.52}             & \textbf{0.279}           & \textbf{0.204}             & \textbf{0.29}                 & \textbf{0.037}              & \textbf{0.443}              & \textbf{0.619}           & \textbf{0.293}              & \textbf{0.341}                   & \textbf{0.513}                     & \textbf{0.857}             & \textbf{0.322}           & \textbf{0.828}              & \textbf{0.213}                 \\
% IoUMatch mAP@0.5  & \textbf{0.059}              & \textbf{0.722}          & \textbf{0.607}            & \textbf{0.562}           & \textbf{0.396}            & \textbf{0.102}           & \textbf{0.05}              & \textbf{0.179}                & \textbf{0.006}              & \textbf{0.16}               & \textbf{0.355}           & \textbf{0.076}              & \textbf{0.216}                   & \textbf{0.047}                     & \textbf{0.672}             & 0.131                    & \textbf{0.676}              & \textbf{0.055} \\ \hline   
% \end{tabular}
% \end{adjustbox}
% \end{table}
